EfficientQAT: Efficient Quantization-Aware Training for Large Language Models

Large language models (LLMs) are crucial in modern natural language processing and artificial intelligence. However, they face challenges in managing their significant memory requirements. Although quantization-aware training (QAT) offers a solution by reducing memory consumption through low-bit representations with minimal accuracy loss, it is impractical due to substantial training resources. To address this, we propose Efficient Quantization-Aware Training (EfficientQAT), a more feasible QAT algorithm. EfficientQAT involves two consecutive phases: Block-wise training of all parameters (Block-AP) and end-to-end training of quantization parameters (E2E-QP). To the best of our knowledge, Block-AP is the first method to enable direct training of all parameters in a block-wise manner, reducing accuracy loss in low-bit scenarios by enhancing the solution space during optimization. E2E-QP then trains only the quantization parameters (step sizes) end-to-end, further improving the performance of quantized models by considering interactions among all sub-modules. Extensive experiments demonstrate that EfficientQAT outperforms previous quantization methods across a range of models, including base LLMs, instruction-tuned LLMs, and multimodal LLMs, with scales from 7B to 70B parameters at various quantization bits. For instance, EfficientQAT obtains a 2-bit Llama-2-70B model on a single A100-80GB GPU in 41 hours, with less than 3 points accuracy degradation compared to the full precision (69.48 vs. 72.41). Code is available at https://github.com/OpenGVLab/EfficientQAT.

==> figure_text/performance_comparisons.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/quant_comparison.pdf}
    \caption{2-bit quantization comparisons}
    \label{fig:2bit_comparisons}
\end{subfigure}
\hfill
\hfill
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/q_peft_comparison.pdf}
    \caption{Q-PEFT comparisons}
    \label{fig:q_pefy_comparisons}
\end{subfigure}
\caption{\textbf{(a)} EfficientQAT significantly surpasses existing uniform quantization methods, and is either superior to or comparable with vector quantization techniques. 
%
\textbf{(b)} EfficientQAT markedly outperforms existing Q-PEFT methods.}
\vspace{-0.5cm}
\end{figure}

==> figure_text/speed_comparisons.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/speed_comparison.pdf}
    \caption{inference speed comparisons}
    \label{fig:inference_speed_comparisons}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/train_comparisons.pdf}
    \caption{training speed comparisons}
    \label{fig:train_speed_comparisons}
\end{subfigure}
\caption{ \textbf{(a):} This panel shows a speed comparison of vector-matrix multiplications for the \textit{gate\_proj} component of Llama-2-70B. Uniform Quantization proves more hardware-efficient than vector quantization.  \textbf{(b):} EfficientQAT can complet the QAT of 70B models on a single A100 GPU with less time.
}
\vspace{-0.5cm}
\end{figure}

==> figures/3_ablations.tex <==
%##################################################################################################
% overall table of all ablations
\begin{table*}[!th]
\centering
%#################################################
% Algorithm Feature Choice
%#################################################
\subfloat[
    \textbf{Training parameters of FL-PTQ.} Training all parameters in Eq.(\ref{eq:quant}) achieve best PTQ performance.
    \label{tab:ablation_fl_ptq_param}
]{
    \centering
    \begin{minipage}{0.29\linewidth}{
        \begin{center}
            \tablestyle{4pt}{1.05}
            \begin{tabular}{x{45}x{40}}
                Parameters & Wiki PPL \\
                \shline
                 None (RTN) & 6.39 \\
                 $s$ & 6.09 \\
                 $s$,$z$ & 6.09 \\
                 $\mathbf{W}$ & 6.13 \\
                 $s$,$z$,$\mathbf{W}$ & \default{\bf 5.93}\\
            \end{tabular}
    \end{center}}
    \end{minipage}
}
\hspace{1.5em}
%#################################################
% Algorithm Distance Function
%#################################################
\subfloat[
    \textbf{Optimization granularity of FL-PTQ.} Block-wise optimization is the best choice for weight-only quantization.
    \label{tab:ablation_fl_ptq_optim}
]{
    \centering
    \begin{minipage}{0.29\linewidth}{
        \begin{center}
            \tablestyle{4pt}{1.05}
            \begin{tabular}{y{45}x{40}}
                Granularity & Wiki PPL  \\
                \shline
                None (RTN) & 6.39 \\
                1 layer & 6.10 \\
                1 block & \default{\bf 5.93} \\
                2 block & 5.96 \\
                4 block & 6.00 \\
            \end{tabular}
    \end{center}}
    \end{minipage}
}
\hspace{1.5em}
%#################################################
% Algorithm Multihead Aggregation
%#################################################
\subfloat[
    \textbf{Reconstruction loss of FL-PTQ.} Asymmetric loss alleviate error accumulation.
    \label{tab:ablation_fl_ptq_loss}
]{
    \centering
    \begin{minipage}{0.29\linewidth}{
        \begin{center}
            \tablestyle{4pt}{1.05}
            \begin{tabular}{y{80}x{40}}
                Loss & Wiki PPL  \\
                \shline
                None (RTN) & 6.39 \\
                $\lvert\lvert \mathcal{F}(\hat{X})-\mathcal{\hat{F}}(\hat{X})\rvert\rvert$ & 6.00 \\
                $\lvert\lvert \mathcal{F}(X)-\mathcal{\hat{F}}(\hat{X})\rvert\rvert$ & \default{\bf 5.93} \\
                Average of above two & 5.96 \\
                & \\
            \end{tabular}
    \end{center}}
    \end{minipage}
}
\\
\centering
\vspace{.3em}
%#################################################
% PTQ Method
%#################################################
\subfloat[
    \textbf{PTQ methods.} Better quantized model can obtain stronger model after fine-tunings.
    \label{tab:ablation_ptq}
]{
    \centering
    \begin{minipage}{0.33\linewidth}{
        \begin{center}
            \tablestyle{4pt}{1.05}
            \begin{tabular}{y{105}x{48}}
                Method & MMLU Acc. \\
                \shline
                RTN + QAME-FT & 42.06 \\
                OmniQuant v1 + QAME-FT & 43.15 \\
                FL-PTQ + QAME-FT & \default{\bf 44.23} \\
                & \\
                % & \\
            \end{tabular}
    \end{center}}
    \end{minipage}
}
\hspace{1.5em}
% #################################################
% Algorithm Choice
% #################################################
\subfloat[
    \textbf{Training Parameters of QAME-FT.} Training $s$ is enough to achieve comparable performance with less bits per parameter.
    \label{tab:ablation_qame_ft_param}
]
{
    \centering
    \begin{minipage}{0.25\linewidth}{
        \begin{center}
            \tablestyle{4pt}{1.05}
            \begin{tabular}{y{30}x{30}x{48}}
                Parameters & bits & MMLU Acc. \\
                \shline
                LoRA & 16 & 44.15 \\
                $s$ & 3.30 & \default{44.23} \\
                $z$ & 3.50 & {\bf 44.56} \\
                $s,z$ & 3.50 & 43.44 \\
                % & \\
            \end{tabular}
    \end{center}}
    \end{minipage}
}
\hspace{1.5em}
\subfloat[
    \textbf{Group Size.} QAME-FT is robust to group size.
    \label{tab:ablation_group_size}
]
{
    \centering
    \begin{minipage}{0.25\linewidth}{
        \begin{center}
            \tablestyle{4pt}{1.05}
            \begin{tabular}{y{30}x{30}x{48}}
                Group & bits & MMLU Acc. \\
                \shline
                % LoRA & 16 & 44.15 \\
                32 & 3.59 & 44.15 \\
                64 & 3.30 & \default{\bf 44.23} \\
                128 & 3.15 & 44.05   \\
                256 & 3.07 & 43.96 \\
            \end{tabular}
    \end{center}}
    \end{minipage}
}
%#################################################
\caption{\textbf{OmniQuant v2 ablation experiments} using LLaMA-2-7B with W3g64 (INT3 and group size as 64) quantization. (a)-(c) are ablations for FL-PTQ, we train on 128 C4 samples and report the perplexity on WikiText2. (d)-(e) are ablations for QAME-FT, we fine-tuning on Alpaca~\cite{alpaca} and report 5-shot accuracy of MMLU. Our default settings are marked in {\setlength{\fboxsep}{2pt}\colorbox{defaultcolor}{{purple}}}.}
\label{tab:ablations}
\vspace{-1.5em}
\end{table*}
%##################################################################################################

==> figures/ablation_ft_train_pram.tex <==
\begin{table}[!ht]
\caption{\textbf{Ablation study about the proposed QAME-FT in LLaMA-2-7B.} $\dag$ Fine-tuning the quantized models on Alpaca~\cite{alpaca} dataset and report the 5-shot accuracy of MMLU~\cite{mmlu} dataset. $\ddag$ Fine-tuning the quantized models on C4 dataset and report the perplexity of Wikitext2. }
\label{tab:ablation_qame_ft}
\vskip 0.15in
\setlength{\tabcolsep}{1pt}
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
\#Bits & Trainable parameters & bits/weight & MMLU Acc.$^\dag$ & Wiki PPL.$^\ddag$ \\
\midrule
16 (FP) & w/o fine-tuning & 16 & 45.50 & 5.47 \\
\cdashline{1-5}
\multirow{3}{*}{\shortstack{W4g64}}& + train $z$ & 2.50 & 46.73 & 5.60 \\
& + train $s,z$ & 2.50 & 46.58 & 5.60 \\
& \textbf{+ train $s$ (ours)} & \textbf{2.28} & \textbf{48.24} & \textbf{5.60} \\
\midrule
\multirow{3}{*}{\shortstack{W3g64}}& + train $z$ & 3.50 & \textbf{44.56} & 5.93 \\
& + train $s,z$ & 3.50 & 43.33 & 5.92 \\
& \textbf{+ train $s$ (ours)} & \textbf{3.30} & 44.23 & \textbf{5.92} \\
\midrule
\multirow{3}{*}{\shortstack{W2g64}}& + train $z$ & 4.50 & 35.01 & 7.70 \\
& + train $s,z$ & 4.50 & 33.27 & 7.68 \\
& \textbf{+ train $s$ (ours)} & \textbf{4.31} & \textbf{35.37} & \textbf{7.67} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> figures/ablation_ptq.tex <==
\begin{table}[!ht]
\caption{Ablation study about the impact of PTQ in the overall pipeline of OmniQuant v2. We maintain the overall pipeline of OmniiQuant v2 and just replace the proposed FL-PTQ with simple rounding-to-nearest(RTN) and previous SoTA method OmniQuant v1~\cite{omniquant}. We finetune the quantized models on Alpaca~\cite{alpaca} dataset and report the 5-shot accuracy of MMLU~\cite{mmlu} dataset. }
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccr}
\toprule
\#Bits & PTQ Method & MMLU Acc. \\
\midrule
\multirow{3}{*}{\shortstack{W4g64}} & RTN & 48.01 & \\
 & OmniQuant v1 & 48.20 \\
 & \textbf{FL-PTQ (ours)} & \textbf{48.24} & \\
\midrule
\multirow{3}{*}{\shortstack{W3g64}} & RTN & 42.06 & \\
 & OmniQuant v1 & 43.15 \\
 & \textbf{FL-PTQ (ours)} & \textbf{44.23} & \\
\midrule
\multirow{3}{*}{\shortstack{W2g64}} & RTN & 27.27 & \\
 & OmniQuant v1 & 31.13 \\
 & \textbf{FL-PTQ (ours)} & \textbf{35.08} & \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> figures/ablation_ptq_train_param.tex <==
\begin{table}[!ht]
\caption{\textbf{Ablation study about training parameters of the proposed FL-PTQ in LLaMA-2-7B.} We only execute PTQ on 128 2048-tokens samples from C4 and report the perplexity in C4 and WikiText2 following existing works~\cite{omniquant,gptq}.}
\label{tab:ablation_fl_ptq}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
\#Bits & Method & Wiki & C4 & Avg. \\
\midrule
\multirow{3}{*}{\shortstack{W4g64}} & RTN & 5.67 & 7.21 & 6.44 \\
\cdashline{2-5}
% & + train $s$ & - & - & - \\
& + train $s,z$ & 5.62 & 7.09 & 6.36 \\
& \textbf{+ train $s,z,V$ (ours)} & 5.62 & 7.08 & 6.35 \\
\midrule
\multirow{3}{*}{\shortstack{W3g64}} & RTN & 6.39 & 8.11 & 7.25 \\
\cdashline{2-5}
% & + train $s$ & - & - & - \\
& + train $s,z$ & 6.09 & 7.53 & 6.81 \\
& \textbf{+ train $s,z,V$ (ours)} & 6.00 & 7.45 & 6.73 \\
\midrule
\multirow{3}{*}{\shortstack{W2g64}} & RTN & 431.98 & 475.33 & 453.66 \\
\cdashline{2-5}
% & + train $s$ & - & - & - \\
& + train $s,z$ & 9.45 & 10.95 & 10.20 \\
& \textbf{+ train $s,z,V$ (ours)} & 8.09 & 9.52 & 8.80 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> figures/alpaca.tex <==


\begin{table*}[t!]
\vspace{-0.5em}
\footnotesize
\centering
\setlength\tabcolsep{2.37pt}
\renewcommand{\arraystretch}{1.15}
  \caption{Llama-1 average MMLU accuracy (5-shot) about instruction-tuning on Alpaca datasets. }\label{tab:q_peft_comparisons}
\begin{tabular}{ccc|cc}
 \toprule
   \bf{Method} & \bf{Bits} & Group & \bf{7B} & \bf{13B}\\
  \midrule
 - & 16 & - & 34.6  & 46.3\\
 \midrule
  PEQA & 4 & -1 & 35.8 & 45.0 \\
  \rowcolor[HTML]{D9D9D9} 
  EfficientQAT & 4 & -1 & \bf{38.8} & \bf{48.2} \\ 
  QLoRA & 4+16 & - & 38.4 & 48.4 \\
  QLoRA w/GPTQ & 4 & 32 & 36.0 & 48.0 \\
  QA-LoRA & 4 & 32 & 39.4 & 49.2 \\
  PEQA & 4 & 64 & 39.4 & 47.4  \\
  IR-QLoRA & 4 & 64 & 40.8 & 49.3 \\
  \rowcolor[HTML]{D9D9D9} 
  EfficientQAT & 4 & 64 & \bf{41.2} & \bf{49.5} \\
  \midrule
  QLoRA w/ GPTQ & 3 & 32 & 34.0 & 46.1 \\
  QA-LoRA & 3 & 32 & 37.4 & 47.3 \\
  IR-QLoRA & 3 & 64 & 38.4 & - \\
  PEQA & 3 & 64 & 38.5 & 46.3  \\
  \rowcolor[HTML]{D9D9D9}
  EfficientQAT & 3 & 64 & \bf{40.0} & \bf{48.2} \\
  \midrule
  QLoRA w/ GPTQ & 2 & 32 & 25.8 & 30.9 \\
  QA-LoRA & 2 & 32 & 27.5 & 36.9 \\
  IR-QLoRA & 2 & 64 & 27.8 & - \\
  PEQA & 2 & 64 & 28.1 & 32.2 \\
  \rowcolor[HTML]{D9D9D9}
  EfficientQAT & 2 & 64 & \bf{32.6} & \bf{40.9} \\
 \bottomrule
\end{tabular}

\end{table*}



==> figures/block_ap_samples.tex <==
\begin{figure}[!t]
    \centering
    \begin{minipage}{0.55\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/train_val_loss_accuracy.pdf}
        \caption{Illustration of training loss, validation loss and average accuracy of w2g64 Llama-2-7b with different training samples size for Block-AP (w/o E2E-QP).}
        \label{fig:train_val_loss}
    \end{minipage}\hfill
    \begin{minipage}{0.43\textwidth}
        \centering
    \caption{Llama-2-7B w2g64 quantization performance with different sample numbers for E2E-QP (w/ Block-AP).}
    \begin{tabular}{c|cc}
    \toprule
    \bf{\# Samples} & \bf{Avg. PPL} & \bf{Avg. Accuracy} \\
    \midrule
    128 & 8.09 & 59.03 \\
    512 & 7.88 & 59.81 \\
    2048 & 7.75 & 60.13 \\
    4096 & 7.68 & 60.14 \\
    8192 & 7.63 & 60.19 \\
    32764 & \textbf{7.50} & \textbf{60.31} \\
    \bottomrule
    \end{tabular}
    \label{tab:e2e_qp_samples}
    \end{minipage}
    \vspace{-0.4cm}
\end{figure}

==> figures/llm_training_details.tex <==
\begin{table}[!ht]
\caption{Training hyperparameters for instruction-tuning of LLM on different dataset and across model size. }
\label{tab:training_details_llm}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lccccccc}
\toprule
Parameters & Dataset & Batch size & LR & Steps & Source Length & Target Length & train on source? \\
\midrule
7B & Alpaca & 16 & 2e-5 & 10000 & 384 & 128 & $\times$ \\
7B & OASST1 & 16 & 2e-5 & 1800 & - & 512 & \checkmark \\
7B & DEITA-10k & 16 & 2e-5 & 1800 & - & 2048 & $\times$ \\
\midrule
13B & Alpaca & 16 & 1e-5 & 10000 & 384 & 128 & $\times$ \\
13B & OASST1 & 16 & 1e-5 & 1800 & - & 512 & \checkmark \\
13B & DEITA-10k & 16 & 1e-5 & 1800 & - & 2048 & $\times$ \\
\midrule
70B & Alpaca & 64 & 1e-5 & 2500 & 384 & 128 & $\times$ \\
70B & OASST1 & 16 & 1e-5 & 1800 & - & 512 & \checkmark \\
70B & DEITA-10k & 16 & 1e-5 & 1800 & - & 2048 & $\times$ \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> figures/method_distinction.tex <==
\begin{table}[!h]
\setlength{\tabcolsep}{1pt}
\caption{Comparison of different memory-efficient fine-tuning methods.$^\dag$ For models with LoRA, we report the bits after merging the LoRA modules into original models.}
\label{tab:relate_work}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{PTQ} & \multirow{2}{*}{LoRA?} & \multicolumn{2}{c}{\#Bit} \\
\cmidrule(l{2pt}r{2pt}){4-5}
& & & Training & Inference$^\dag$ \\
\midrule
QLoRA & NF4 & \checkmark & low-bits+16 & 16 \\
INT2.1 & GPTQ(INT) & \checkmark & low-bits+16 & 16 \\
LQ-LoRA & NF4/3/2 & \checkmark & low-bits+16 & 16 \\
LoftQ & NF4/2 & \checkmark & low-bits+16 & 16 \\
QA-LoRA & GPTQ (INT) & \checkmark & low-bits+16 & low-bits \\
PEQA & RTN (INT) & $\times$ & low-bits & low-bits \\
OmniQuant v2 & FL-PTQ (INT) & $\times$ & low-bits & low-bits \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> figures/mixed_table.tex <==
\begin{table*}[!ht]
    \begin{minipage}[t]{0.50\textwidth}
        \centering
        \vspace{-0.5em}
        \footnotesize
        \caption{Llama-1 average MMLU accuracy (5-shot) about instruction-tuning on Alpaca dataset.}
        \label{tab:q_peft_comparisons}
        \begin{tabular}{ccc|cc}
            \toprule
            \bf{Method} & \bf{Bits} & Group & \bf{7B} & \bf{13B}\\
            \midrule
             - & 16 & - & 34.6  & 46.3\\
             \midrule
              PEQA & 4 & -1 & 35.8 & 45.0 \\
              \rowcolor[HTML]{D9D9D9} 
              EfficientQAT & 4 & -1 & \bf{38.8} & \bf{48.2} \\ 
              QLoRA & 4+16 & - & 38.4 & 48.4 \\
              QLoRA w/GPTQ & 4 & 32 & 36.0 & 48.0 \\
              QA-LoRA & 4 & 32 & 39.4 & 49.2 \\
              PEQA & 4 & 64 & 39.4 & 47.4  \\
              IR-QLoRA & 4 & 64 & 40.8 & 49.3 \\
              \rowcolor[HTML]{D9D9D9} 
              EfficientQAT & 4 & 64 & \bf{41.2} & \bf{49.5} \\
              \midrule
              QLoRA w/ GPTQ & 3 & 32 & 34.0 & 46.1 \\
              QA-LoRA & 3 & 32 & 37.4 & 47.3 \\
              IR-QLoRA & 3 & 64 & 38.4 & - \\
              PEQA & 3 & 64 & 38.5 & 46.3  \\
              \rowcolor[HTML]{D9D9D9}
              EfficientQAT & 3 & 64 & \bf{40.0} & \bf{48.2} \\
              \midrule
              QLoRA w/ GPTQ & 2 & 32 & 25.8 & 30.9 \\
              QA-LoRA & 2 & 32 & 27.5 & 36.9 \\
              IR-QLoRA & 2 & 64 & 27.8 & - \\
              PEQA & 2 & 64 & 28.1 & 32.2 \\
              \rowcolor[HTML]{D9D9D9}
              EfficientQAT & 2 & 64 & \bf{32.6} & \bf{40.9} \\
            \bottomrule
        \end{tabular}
    \end{minipage}%
    \hfill
    \begin{minipage}[t]{0.55\textwidth}
        \centering
        \caption{Effectiveness of each component on Llama-2-7B w2g64 quantization.}
        \label{tab:ablation_components}
        \renewcommand{\arraystretch}{0.7}
        \begin{tabular}{cc|cc}
        \toprule
        \bf{Block-AP} & \bf{E2E-QP} & \bf{Avg. PPL} & \bf{Avg. Accuracy} \\
        \midrule
        \XSolidBrush & \XSolidBrush & 453.49 & 40.69 \\
         \checkmark   & \XSolidBrush  & 8.53 & 58.99 \\ 
          \XSolidBrush  & \checkmark   & 9.33 & 55.71 \\ 
          \checkmark  & \checkmark   & 7.68 &  60.14 \\ 
        \bottomrule
        \end{tabular}
        
        % \vspace{1em} % 调整表格间距
        
        \caption{W2g64 Llama-2-7B performance with different trainable parameters in the block-wise training (w/o E2E-QP). ``\# Param.'' indicates trainable parameters count in a block.}
        \label{tab:ptq_variants_comparisons}
        \tabcolsep=0.05cm
        \begin{tabular}{c|cccc}
        \toprule
        \bf{Param.} & \bf{\# Param.} & \bf{Memory} & \bf{Avg. PPL} & \bf{Avg. Accuracy} \\
        \midrule
        clipping & 6.3M & 6.4GB & 11.28 & 53.20 \\
        $s$,$z$ & 6.3M & 6.4GB & 10.26 & 55.20 \\
        round & 202.4M & 8.6GB & 15.50 & 45.32 \\
        $s$,$z$,round &  208.7M & 9.3GB & 9.17 & 57.14 \\
        $s$,$z$,$\mathbf{W}$ & 208.7M & 8.5GB  & 8.53 & 58.99 \\
        \bottomrule
        \end{tabular}
        
        % \vspace{1em} % 调整表格间距
        
        \caption{Llama-2-7B w2g64 quantization with different trainable parameters for E2E-QP (w/ Block-AP).}
        \label{tab:e2e-ft-variants}
        \begin{tabular}{c|ccc}
        \toprule
        \bf{Param.} & \bf{Avg. Bits} & \bf{Avg. PPL} & \bf{Avg. Accuracy} \\
        \midrule
        $s$ & 2.28 & 7.68 & 60.14 \\
        $z$ & 2.50 & 7.69 & 60.08 \\
        $s,z$ & 2.50 & 7.68 & 60.18 \\
        \bottomrule
        \end{tabular}
    \end{minipage}
\vspace{-0.5cm}
\end{table*}

==> figures/mmlu_mtbench_comparisons.tex <==
\begin{table*}[!ht]
\renewcommand{\arraystretch}{0.60}
\caption{\textbf{MMLU and MTbench Results about instruction tuning of large language models.}  Note that the MTBench scores are estimated through `gpt-3.5-turbo-1106'. `QLoRA + FL-PTQ' indicates that we leverage proposed FL-PTQ to quantized the QLoRA models into low-bits for fair comparisons, and the {\color{blue}{blue}} numbers indicate the performance benefits of OmniQuant v2 compared with `QLoRA + FL-PTQ'.  }
\label{tab:mmlu_mtbench_comparisons}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lccccll}
\toprule
\multirow{2}{*}{Base Model} & \multirow{2}{*}{Method} & \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{\#Bit}  &  MMLU (5-shot) & MTBench \\
\cmidrule(l{2pt}r{2pt}){4-5}
& & & Training & Inference & Acc. (\%) & Score \\
% Base Model & Method & Dataset & Training \#Bit & Inference \#Bit & MMLU Acc. (5-shot) (\%) & MTBench Score \\
\midrule
\multirow{23}{*}{\shortstack{LLaMA-2-7B}} & w/o fingtuning & - & 16 & 16 & 45.50 & 1.48 \\
\cdashline{2-7}
% \multirow{23}{*}{\shortstack{LLaMA-2-7B}} & LoRA & - & 16 & - & - \\
% & QLoRA & \multirow{8}{*}{\shortstack{Alpaca}} & 4+16 & 46.30 & \textcolor{red}{4.56} \\
& QLoRA & Alpaca & 4+16 & 16 & 46.30 & 4.76 \\
& QALoRA & Alpaca & 4+16 & 4 & 43.90 & - \\
& QLoRA + FL-PTQ & Alpaca & 4+16 & 4 & 44.58 & 4.75 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}Alpaca & \cellcolor{Gray}4 & \cellcolor{Gray}4 &  \cellcolor{Gray}\textbf{48.24}{\color{blue}(+3.66)} &  \cellcolor{Gray}\textbf{4.80}{\color{blue}(+0.05)} \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 3 & 41.93 & 4.50 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}Alpaca & \cellcolor{Gray}3 & \cellcolor{Gray}3 &  \cellcolor{Gray}\textbf{44.23}{\color{blue}(+2.30)} &  \cellcolor{Gray}\textbf{4.73}{\color{blue}(+0.23)} \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 2 & 30.82 & 3.54 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}Alpaca & \cellcolor{Gray}2 & \cellcolor{Gray}2 &  \cellcolor{Gray}\textbf{35.08}{\color{blue}(+4.25)} &  \cellcolor{Gray}\textbf{4.28}{\color{blue}(+0.74)} \\
\cdashline{2-7}
% & QLoRA & \multirow{7}{*}{\shortstack{OASST1}} & 4+16 & 46.99 & 6.34 \\
& QLoRA & OASST1 & 4+16 & 16 & 46.99 & 6.34 \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 4 & 46.24 & 6.17 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}OASST1 & \cellcolor{Gray}4 & \cellcolor{Gray}4 &  \cellcolor{Gray}\textbf{44.62}{\color{blue}(-1.62)} &  \cellcolor{Gray}\textbf{6.46}{\color{blue}(+0.29)} \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 3 & 43.49 & 5.77 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}OASST1 & \cellcolor{Gray}3 & \cellcolor{Gray}3 &  \cellcolor{Gray}\textbf{43.33}{\color{blue}(-0.16)} &  \cellcolor{Gray}\textbf{6.18}{\color{blue}(+0.41)} \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 2 & 28.50 & 3.35 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}OASST1 & \cellcolor{Gray}2 & \cellcolor{Gray}2 &  \cellcolor{Gray}\textbf{34.24}{\color{blue}(+5.74)} &  \cellcolor{Gray}\textbf{5.34}{\color{blue}(+1.99)} \\
\cdashline{2-7}
& QLoRA & DEITA-10k & 4+16 & 16 & 46.81 & 6.67 \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 4 & 46.32 & 6.32 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}4 & \cellcolor{Gray}4 &  \cellcolor{Gray}\textbf{46.90}{\color{blue}(+0.58)} &  \cellcolor{Gray}\textbf{6.76}{\color{blue}(+0.44)} \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 3 & 44.22 & 6.07 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}3 & \cellcolor{Gray}3 &  \cellcolor{Gray}\textbf{45.99}{\color{blue}(+1.77)} &  \cellcolor{Gray}\textbf{6.86}{\color{blue}(+0.79)} \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 2 & 29.30 & 3.25 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}2 & \cellcolor{Gray}2 &  \cellcolor{Gray}\textbf{36.52}{\color{blue}(+7.22)} &  \cellcolor{Gray}\textbf{5.88}{\color{blue}(+2.63)} \\
\midrule
\multirow{23}{*}{\shortstack{LLaMA-2-13B}} & w/o fingtuning & - & 16 & 16 & 55.30 & 1.50 \\
% \multirow{23}{*}{\shortstack{LLaMA-2-13B}} & LoRA & - & 16 & - & - \\
\cdashline{2-7}
% & QLoRA & \multirow{8}{*}{\shortstack{Alpaca}} & 4+16 & 52.06 & 6.01 \\
& QLoRA & Alpaca & 4+16 & 16 & 52.06 & 6.01 \\
& QALoRA & Alpaca & 4+16 & 4 & 51.70 & - \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 4 & 51.50 & 5.99 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}Alpaca & \cellcolor{Gray}4 & \cellcolor{Gray}4 &  \cellcolor{Gray}\textbf{53.02}{\color{blue}(+1.52)} &  \cellcolor{Gray}\textbf{6.00}{\color{blue}(+0.01)} \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 3 & 50.17 & 6.01 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}Alpaca & \cellcolor{Gray}3 & \cellcolor{Gray}3 &  \cellcolor{Gray}\textbf{53.68}{\color{blue}(+3.51)} &  \cellcolor{Gray}\textbf{6.14}{\color{blue}(+0.13)} \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 2 & 43.20 & 4.84 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}Alpaca & \cellcolor{Gray}2 & \cellcolor{Gray}2 &  \cellcolor{Gray}\textbf{48.11}{\color{blue}(+5.91)} &  \cellcolor{Gray}\textbf{5.51}{\color{blue}(+0.65)}\\
\cdashline{2-7}
& QLoRA & OASST1 & 4+16 & 16 & 54.44 & 6.81 \\
& QLoRA + FL-PTQ &  OASST1 & 4+16 & 4 & 54.32 & 6.69 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}OASST1 & \cellcolor{Gray}4 & \cellcolor{Gray}4 &  \cellcolor{Gray}\textbf{54.15}{\color{blue}(-0.17)} &  \cellcolor{Gray}\textbf{6.76}{\color{blue}(+0.07)} \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 3 & 52.56 & 6.18 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}OASST1 & \cellcolor{Gray}3 & \cellcolor{Gray}3 &  \cellcolor{Gray}\textbf{53.55}{\color{blue}(+0.98)} &  \cellcolor{Gray}\textbf{6.57}{\color{blue}(+0.39)} \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 2 & 42.01 & 3.67 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray} OASST1 & \cellcolor{Gray}2 & \cellcolor{Gray}2 &  \cellcolor{Gray}\textbf{46.52}{\color{blue}(+4.51)} &  \cellcolor{Gray}\textbf{5.90}{\color{blue}(+2.23)} \\
\cdashline{2-7}
& QLoRA & DEITA-10k & 4+16 & 16 & 55.11 & 6.67 \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 4 & 54.54 & 6.60 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}4 & \cellcolor{Gray}4 &  \cellcolor{Gray}\textbf{55.33}{\color{blue}(-0.78)} &  \cellcolor{Gray}\textbf{7.16}{\color{blue}(+0.56)} \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 3 & 52.55 & 6.53 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}3 & \cellcolor{Gray}3 &  \cellcolor{Gray}\textbf{54.93}{\color{blue}(+2.38)} &  \cellcolor{Gray}\textbf{6.80}{\color{blue}(+0.27)} \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 2 & 40.04 & 4.57 \\
&  \cellcolor{Gray}\textbf{OmniQuant v2} &  \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}2 & \cellcolor{Gray}2 &  \cellcolor{Gray}\textbf{48.44}{\color{blue}(+8.40)} &  \cellcolor{Gray}\textbf{6.17}{\color{blue}(+1.60)} \\
\midrule
\multirow{23}{*}{\shortstack{LLaMA-2-70B}} & w/o fingtuning & - & 16 & 16 & 68.84 & 1.75 \\
% \multirow{23}{*}{\shortstack{LLaMA-2-70B}} & LoRA & - & 16 & - & - \\
\cdashline{2-7}
& QLoRA & Alpaca & 4+16 & 16 & 65.81 & 5.68 \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 4 & 65.53 & 5.65 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}Alpaca & \cellcolor{Gray}4 & \cellcolor{Gray}4 & \cellcolor{Gray}\textbf{66.44}{\color{blue}(+0.91)} & \cellcolor{Gray}\textbf{5.76}{\color{blue}(+0.11)} \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 3 & 65.10 & 5.42 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}Alpaca & \cellcolor{Gray}3 & \cellcolor{Gray}3 & \cellcolor{Gray}\textbf{66.88}{\color{blue}(+1.78)} & \cellcolor{Gray}\textbf{5.63}{\color{blue}(+0.21)} \\
& QLoRA + FL-PTQ & Alpaca & 4+16& 2 & 59.12 & 4.88 \\
& \textbf{OmniQuant v2} & \cellcolor{Gray}Alpaca & \cellcolor{Gray}2 & \cellcolor{Gray}2 & \cellcolor{Gray}\textbf{61.83}{\color{blue}(+2.71)} & \cellcolor{Gray}\textbf{5.57}{\color{blue}(+0.69)} \\
\cdashline{2-7}
& QLoRA & OASST1 & 4+16 & 16 & 68.91 & 7.17 \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 4 & 68.71 & 6.98 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}OASST1 & \cellcolor{Gray}4 & \cellcolor{Gray}4 & \cellcolor{Gray}\textbf{68.55}{\color{blue}(-0.16)} & \cellcolor{Gray}\textbf{7.17}{\color{blue}(+0.19)} \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 3 & 68.12 & 6.87 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}OASST1 & \cellcolor{Gray}3 & \cellcolor{Gray}3 & \cellcolor{Gray}\textbf{68.23}{\color{blue}(+0.11)} & \cellcolor{Gray}\textbf{7.03}{\color{blue}(+0.16)} \\
& QLoRA + FL-PTQ & OASST1 & 4+16 & 2 & 60.46 & 5.88 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}OASST1 & \cellcolor{Gray}2 & \cellcolor{Gray}2 & \cellcolor{Gray}\textbf{63.20}{\color{blue}(+2.74)} & \cellcolor{Gray}\textbf{6.76}{\color{blue}(+0.88)} \\
\cdashline{2-7}
& QLoRA & DEITA-10k & 4+16 & 16 & 68.25 & 7.58 \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 4 & 67.93 & 7.40 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}4 & \cellcolor{Gray}4 & \cellcolor{Gray}\textbf{67.86}{\color{blue}(-0.07)} & \cellcolor{Gray}\textbf{7.73}{\color{blue}(+0.33)} \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 3 & 66.66 & 7.35 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}3 & \cellcolor{Gray}3 & \cellcolor{Gray}\textbf{67.68}{\color{blue}(+1.02)} & \cellcolor{Gray}\textbf{7.76}{\color{blue}(+0.41)} \\
& QLoRA + FL-PTQ & DEITA-10k & 4+16 & 2 & 60.43 & 6.35 \\
& \cellcolor{Gray}\textbf{OmniQuant v2} & \cellcolor{Gray}DEITA-10k & \cellcolor{Gray}2 & \cellcolor{Gray}2 & \cellcolor{Gray}\textbf{63.58}{\color{blue}(+3.12)} & \cellcolor{Gray}\textbf{7.03}{\color{blue}(+0.68)} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> figures/ppl_2048_backup.tex <==
\begin{table*}[ht]
\caption{Llama 2 \& 3 Wikitext2 and C4 perplexity ($\downarrow$), context length 2048.}
\label{tab:ppl2048}
\centering
% \small\sc
\tabcolsep=0.15cm
\begin{tabular}{@{}cccc|ccccc|ccccc@{}}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{5}{c}{Wikitext 2}& \multicolumn{5}{c}{C4}\\ \midrule
Method& Bits& Type & \multicolumn{1}{c|}{Group} & 2-7 & 2-13& 2-70 & 3-8 &\multicolumn{1}{c|}{3-70} & 2-7 & 2-13& 2-70 & 3-8 & 3-70\\ \midrule
FP16 & 16 & - & \multicolumn{1}{c|}{16} & 5.47& 4.88& 3.32& - & \multicolumn{1}{c|}{-} & 6.97& 6.47& 5.52 & - & -\\
\rowcolor[HTML]{D9D9D9} 
AWQ & 4 & uniform & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}128} & 6.15& 5.12& - & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & 7.68& 6.74& - & - & - \\
\rowcolor[HTML]{D9D9D9} 
OmniQ& 4 & uniform & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}128} & 5.74& 5.02& 3.47 & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-}& 7.35& 6.65& 5.65 & - & - \\
\rowcolor[HTML]{D9D9D9} 
AQLM & 4 & vector & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & - & - & - & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & - & - & - & - & - \\
\rowcolor[HTML]{D9D9D9} 
QuIP\#& 4 & vector & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & 5.56 & 4.95 & 3.38 & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & 7.07 & 6.54 & 5.56 & - & - \\
\rowcolor[HTML]{D9D9D9} 
EfficientQAT & 4 & uniform & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}128} & - & - & - & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & - & - & - & - & - \\
AWQ& 3& uniform & \multicolumn{1}{c|}{128} & 24.0& 10.5 & - & - &\multicolumn{1}{c|}{-} & 23.9& 13.1& -  & - & -\\
OmniQ& 3& uniform & \multicolumn{1}{c|}{128} & 6.58& 5.58& 3.92 & - & \multicolumn{1}{c|}{-}& 8.65& 7.44& 6.06 & - & -\\
AQLM & 3 & vector & \multicolumn{1}{c|}{-} & - & - & - & - & \multicolumn{1}{c|}{-} & - & - & - & - & - \\
QuIP\#& 3& vector & \multicolumn{1}{c|}{-} & 5.79 & 5.10 & 3.56 & - & \multicolumn{1}{c|}{-}& 7.32 & 6.72 & 5.67 & - & - \\
EfficientQAT & 3 & uniform & \multicolumn{1}{c|}{128} & - & - & - & - & \multicolumn{1}{c|}{-} & - & - & - & - & - \\
\rowcolor[HTML]{D9D9D9} 
OmniQ& 2 & uniform & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}128} & 37.4& 17.2 & 7.81 & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-}& 90.6& 26.8& 12.3 & - & -\\
\rowcolor[HTML]{D9D9D9} 
AQLM & 2 & vector & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & - & - & - & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & - & - & - & - & - \\
\rowcolor[HTML]{D9D9D9} 
QuIP\#& 2 & vector & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & 6.66 & 5.74 & 4.16 & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & 8.35 & 7.45 & 6.12 & - & - \\
\rowcolor[HTML]{D9D9D9} 
EfficientQAT & 2 & uniform & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}128} & - & - & - & - & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}-} & - & - & - & - & - \\
\bottomrule
\end{tabular}
\end{table*}

==> figures/ptq_comparisons.tex <==
\begin{table*}[!ht]
\caption{\textbf{Comparisons about proposed FL-PTQ with previous uniform quantization methods.} We execute quantization on 128 2048-tokens samples from C4 and report the perplexity in C4 and WikiText2.}
\label{tab:ptq_comparisons}
\vskip 0.15in

\begin{subtable}{\textwidth}
\begin{center}
\caption{Results for group sizes 64}
\begin{small}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{W4g64} & \multicolumn{3}{c}{W3g64} & \multicolumn{3}{c}{W2g64} \\
\cmidrule(l{2pt}r{2pt}){3-5}
\cmidrule(l{2pt}r{2pt}){6-8}
\cmidrule(l{2pt}r{2pt}){9-11}
& & Wiki & C4 & Avg. & Wiki & C4 & Avg. & Wiki & C4 & Avg. \\
\midrule
\multirow{5}{*}{LLaMA-2-7B} & RTN & 5.67 & 7.21 & 6.44 & 6.39 & 8.11 & 7.25 & 431.98 & 475.33 & 453.66 \\
 & GPTQ & 5.58 & 7.08 & \bf6.33 & 6.16 & 7.66 & 6.91 & 22.67 & 19.52 & 21.10 \\
 & AWQ & 5.59 & 7.10 & 6.35 &  6.11 & 7.68 & 6.90 & 2.1e5 & 1.6e5 & 1.9e5 \\
 & OmniQuant v1 & 5.59 & 7.10 & 6.35 & 6.11 & 7.63 & 6.87 & 10.55 & 12.24 & 11.40 \\
 & \cellcolor{Gray}FL-PTQ (ours) & \cellcolor{Gray}5.59 & \cellcolor{Gray}7.07 & \cellcolor{Gray}\bf6.33  & \cellcolor{Gray}5.93 & \cellcolor{Gray}7.40 & \cellcolor{Gray}\bf6.67  & \cellcolor{Gray}8.11 & \cellcolor{Gray}9.44 & \cellcolor{Gray}\bf8.77 \\
\midrule
\multirow{5}{*}{LLaMA-2-13B} & RTN & 4.97 & 6.56 & 5.77 & 5.38 & 7.02 & 6.20 & 26.22 & 28.69 & 27.46 \\
 & GPTQ & 4.96 & 6.53 & \bf5.75 & 5.28 & 6.86 & 6.07 & 20.05 & 13.57 & 16.81 \\
 & AWQ & 4.96 & 6.55 & 5.76 & 5.25 & 6.88 & 6.06 & 1.2e5 & 9.5e4 & 1.1e5 \\
 & OmniQuant v1 & 4.96 & 6.55 & 5.76 & 5.27 & 6.87 & 6.07 & 8.06 & 9.85 & 8.96 \\
 & \cellcolor{Gray}FL-PTQ (ours) & \cellcolor{Gray}4.97 & \cellcolor{Gray}6.53 & \cellcolor{Gray}\bf5.75 & \cellcolor{Gray}5.23 & \cellcolor{Gray}6.77 & \cellcolor{Gray}\bf6.00 & \cellcolor{Gray}6.89 & \cellcolor{Gray}8.33 & \cellcolor{Gray}\bf7.61 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\caption{Results for group sizes 128}
\end{subtable}
\vspace{1em}
\begin{subtable}{\textwidth}
\begin{center}
\begin{small}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{W4g128} & \multicolumn{3}{c}{W3g128} & \multicolumn{3}{c}{W2g128} \\
\cmidrule(l{2pt}r{2pt}){3-5}
\cmidrule(l{2pt}r{2pt}){6-8}
\cmidrule(l{2pt}r{2pt}){9-11}
& & Wiki & C4 & Avg. & Wiki & C4 & Avg. & Wiki & C4 & Avg. \\
\midrule
\multirow{5}{*}{LLaMA-2-7B} & RTN & 5.72 & 7.24 & 6.48 & 6.66 & 8.40 & 7.53 & 4.2e3 & 4.9e3 & 4.6e3 \\
 & GPTQ & 5.61 & 7.12 & 6.37 & 6.29 & 7.89 & 7.09 & 36.77 & 33.70 & 35.24  \\
 & AWQ & 5.62 & 7.13 & 6.38 & 6.24 & 7.84 & 7.04 & 2.2e5 & 1.7e5& 2.0e5 \\
 & OmniQuant v1 & 5.58 & 7.12 & 6.35 & 6.03 & 7.75 & 6.89 & 11.06 & 15.02 & 13.04  \\
 & \cellcolor{Gray}FL-PTQ (ours) & \cellcolor{Gray}5.60 & \cellcolor{Gray}7.08 & \cellcolor{Gray}\bf6.34 & \cellcolor{Gray}6.02 & \cellcolor{Gray}7.46 & \cellcolor{Gray}\bf6.74 & \cellcolor{Gray}8.61 & \cellcolor{Gray}10.05 & \cellcolor{Gray}\bf9.33  \\
\midrule
\multirow{5}{*}{LLaMA-2-13B} & RTN & 4.98 & 6.58 & 5.78 & 5.51 & 7.18 & 6.35 & 122.08 & 139.65 & 130.87  \\
 & GPTQ & 4.98 & 6.56 & 5.77 & 5.42 & 7.00 & 6.21 & 28.14 & 20.97 & 24.56  \\
 & AWQ & 4.97 & 6.56 & \bf5.76 & 5.32 & 6.94 & 6.13  & 1.2e5 & 9.4e4 & 1.1e5 \\
 & OmniQuant v1 & 4.95 & 6.56 & \bf5.76 & 5.28 & 6.98 & 6.13 & 8.26 & 11.05 & 9.67  \\
 & \cellcolor{Gray}FL-PTQ (ours) & \cellcolor{Gray}4.97 & \cellcolor{Gray}6.54 & \cellcolor{Gray}\bf5.76 & \cellcolor{Gray}5.27 & \cellcolor{Gray}6.80 & \cellcolor{Gray}\bf6.04 & \cellcolor{Gray}7.19 & \cellcolor{Gray}8.62 & \cellcolor{Gray}\bf7.90  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{subtable}
\vspace{1em}
\begin{subtable}{\textwidth}
\begin{center}
\caption{Results for channel-wise}
\begin{small}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{W4g-1} & \multicolumn{3}{c}{W3g-1} & \multicolumn{3}{c}{W2g-1} \\
\cmidrule(l{2pt}r{2pt}){3-5}
\cmidrule(l{2pt}r{2pt}){6-8}
\cmidrule(l{2pt}r{2pt}){9-11}
& & Wiki & C4 & Avg. & Wiki & C4 & Avg. & Wiki & C4 & Avg. \\
\midrule
\multirow{5}{*}{LLaMA-2-7B} & RTN & 6.11 & 7.71 & 6.91 & 539.48 & 402.35 & 470.91 & 3.8e4 & 7.2e4 & 5.5e4 \\
 & GPTQ & 5.83 & 7.37 & 6.60 & 8.37 & 9.81 & 9.09 & 7.7e3 & 323.12 & 4.0e3  \\
 & AWQ & 6.15 & 7.68 & 6.92 & 24.00 & 23.85 & 23.93 & - & - & - \\
 & OmniQuant v1 & 5.74 & 7.35 & 6.55 & 6.58 & 8.65 & 7.62 & 37.37 & 26.76 & 32.07  \\
 & \cellcolor{Gray}FL-PTQ (ours) & \cellcolor{Gray}5.73 & \cellcolor{Gray}7.19 & \cellcolor{Gray}\bf6.46 &  \cellcolor{Gray}6.49 & \cellcolor{Gray}7.91 & \cellcolor{Gray}\bf7.20 & \cellcolor{Gray}18.85 & \cellcolor{Gray}15.72 & \cellcolor{Gray}\bf17.28  \\
\midrule
\multirow{5}{*}{LLaMA-2-13B} & RTN & 5.20 & 6.83 & 6.02 & 10.68 & 12.51 & 11.59 & 5.6e4 & 7.2e4 & 6.4e4  \\
 & GPTQ & 5.13 & 6.70 & 5.92 & 6.44 & 8.02 & 7.23 & 2.1e3 & 323.12 & 1.2e3  \\
 & AWQ & 5.12 & 6.74 & 5.93 & 10.45 & 13.07 & 11.76 & - & - & - \\
 & OmniQuant v1 & 5.02 & 6.65 & 5.84 & 5.58 & 7.44 & 6.51 & 17.21 & 26.76 & 21.98  \\
 & \cellcolor{Gray}FL-PTQ (ours) & \cellcolor{Gray}5.03 & \cellcolor{Gray}6.58 & \cellcolor{Gray}\bf5.80 & \cellcolor{Gray}5.58 & \cellcolor{Gray}7.00 & \cellcolor{Gray}\bf6.29 & \cellcolor{Gray}11.59 & \cellcolor{Gray}10.78 & \cellcolor{Gray}\bf11.18  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{subtable}
\vskip -0.1in
\end{table*}

==> figures/qat_comparisons.tex <==
% \begin{wraptable}{r}{0.56\textwidth}
% \vspace{-0.5cm}
\begin{table}[!ht]
  \caption{Comparison with QAT methods on Llama-2 \& 3 models.}
    \tabcolsep=0.01cm
    \begin{tabular}{cccc|ccc}
    \toprule
    \multirow{2}{*}{\bf{Model}} & \multirow{2}{*}{\bf{Method}} &\multirow{2}{*}{\bf{Bits}} & \multirow{2}{*}{\bf{Group}} & \multicolumn{2}{c}{PPL} & Average \\
    \cmidrule(l{2pt}r{2pt}){5-6}
    & & & & Wiki & C4 & Accuracy \\
    \midrule
    2-7B & LLM-QAT & 3 & 128 & 6.02 & - & - \\
    2-7B & BitDistiller & 3 & 128 & 5.97 & - & - \\
    \rowcolor[HTML]{D9D9D9} 
    2-7B & EfficientQAT & 3 & 128 & \bf{5.81} & \bf{7.34} & \bf{64.02} \\
    \midrule
    2-7B & PB-LLN & 2 & 64 & 20.37 & 44.88 & 37.59 \\
    2-7B & DB-LLN &  2 & 64 & 7.23 & 9.62 & 55.12 \\
    2-7B & EfficientQAT & 2 & 64 & 6.86 & 8.50 & 60.14 \\
    \midrule
    2-7B & LLM-QAT & 2 & 128 & 9.30 & - & - \\
    2-7B & BitDistiller & 2 & 128 & 8.08 & - & - \\
    \rowcolor[HTML]{D9D9D9} 
    2-7B & EfficientQAT & 2 & 128 & \bf{7.19} & \bf{8.79} & \bf{59.50} \\
    \midrule
    3-8B & PB-LLM & 2 & 128 & 24.70 & 79.20 & 38.80 \\
    3-8B & DB-LLM & 2 & 128 & 13.60 & 19.20 & 51.80 \\
    \rowcolor[HTML]{D9D9D9} 
    3-8B & EfficientQAT & 2 & 128 & \bf{9.80} & \bf{13.22} & \bf{59.37} \\
    \midrule
    3-70B & PB-LLM & 2 & 128 & 11.60 & 34.50 & 46.00 \\
    \rowcolor[HTML]{D9D9D9}
    3-70B & EfficientQAT & 2 & 128 & \bf{6.07} & \bf{9.23} & \bf{67.57} \\
    \midrule
    \end{tabular}
    \label{tab:qat_comparisons}
    % \vspace{-0.9cm}
% \end{wraptable}
\end{table}


==> figures/zero_shot_acc_4bit.tex <==


\begin{table*}[!ht]
\vspace{-0.5em}
\footnotesize
\centering
\setlength\tabcolsep{2.37pt}
\renewcommand{\arraystretch}{1.15}
  \caption{4-bit Llama 2 \& 3 zero-shot accuracy by lm\_eval v0.4.2 ( acc is reported, not acc\_norm ) }\label{tab:4bit_acc}
\begin{tabular}{lccc|cccccc}
 \toprule
  \bf{Model} & \bf{Method} & \bf{Bits} & Group & \bf{WinoGrande} & \bf{HellaSwag}  & \bf{ArcC} & \bf{ArcE}  & \bf{PiQA} & \bf{Average accuracy$\uparrow$}\\
  \midrule
  \multirow{8}{*}{2-7B} & -  & - & 16 & 69.22 & 57.16 & 43.52 & 76.26 & 78.07 & 64.85 \\
  & RTN  & 4 & 128  & 68.35 & 56.91 & 43.52 & 76.26 & 77.58 & 64.52  \\
  & GPTQ  & 4 & 128  & 69.06 & 56.36 & 42.15 & 75.63 & 78.02 & 64.24  \\
  & AWQ & 4 & 128 & 68.98 & 56.40 & 43.86 & 76.14 & 77.31 & 64.54  \\
  & OmniQ & 4 & 128 & 68.98  & 56.59  & 43.34  & 75.76  & 77.91  & 64.52  \\ 
  & AutoRound & 4 & 128 & 68.67  & 56.79  & 42.58  & 75.76  & 78.13  & 64.39  \\ 
  & QuIP\# & 4 & - & 69.22  & 56.65  & 43.00  & 75.51  & 78.02 & 64.48  \\ 
    \rowcolor[HTML]{D9D9D9} 
  & EfficientQAT & 4 & 128 & 69.22  & 57.00  & 42.32  & 75.13  & 77.69 & 64.27  \\ 
 \midrule
  \multirow{8}{*}{2-13B} & - & 16 & - & 72.22  & 60.07  & 48.29  & 79.42  & 79.05  & 67.81 \\
  & RTN  & 4 & 128  & 72.14  & 59.77  & 47.95  & 79.00  & 78.62  & 67.50  \\
  & GPTQ  & 4 & 128  & 72.14  & 59.76  & 47.53  & 78.58  & 78.35  & 67.27  \\
  & AWQ & 4 & 128 & 73.32  & 59.80  & 46.50  & 79.38  & 79.05  & 67.61  \\
  & OmniQ & 4 & 128 & 72.06  & 59.53  & 47.18  & 78.37  & 78.35  & 67.10  \\ 
  & AutoRound & 4 & 128 & 71.67  & 59.87  & 47.01  & 79.25  & 79.00  & 67.36  \\ 
  & QuIP\# & 4 & - & 72.69  & 59.49  & 46.59  & 78.62  & 79.00 & 67.28  \\ 
    \rowcolor[HTML]{D9D9D9} 
  & EfficientQAT & 4 & 128 & 71.98  & 59.87  & 47.53  & 79.34  & 78.89 & 67.52  \\ 
 \midrule
  \multirow{8}{*}{2-70B} & - & 16 & - & 77.98  & 64.77  & 54.44  & 82.70  & 82.15  & 72.41 \\
  & RTN  & 4 & 128  & 78.14  & 63.93  & 54.78  & 82.79  & 81.66  & 72.26  \\
  & GPTQ  & 4 & 128  & 78.22  & 64.45  & 54.61  & 82.79  & 81.88  & 72.39  \\
  & AWQ & 4 & 128 & 77.58  & 64.48  & 55.12  & 82.70  & 82.32  & 72.44  \\
  & OmniQ & 4 & 128 & 77.51  & 64.52  & 55.12  & 82.91  & 81.88  & 72.39  \\ 
  & AutoRound & 4 & 128 & 78.30  & 64.60  & 54.52  & 82.87  & 82.05  & 72.47  \\ 
  & QuIP\# & 4 & - & 77.82  & 64.51  & 54.44  & 82.37  & 81.72 & 72.17  \\ 
    \rowcolor[HTML]{D9D9D9} 
  & EfficientQAT & 4 & 128 & 78.45  & 64.57  & 55.12  & 83.00  &81.94  & 72.62  \\ 
 \midrule
  \multirow{5}{*}{3-8B} & - & - & 16 & 72.61  & 60.17  & 50.43  & 80.09  & 79.60  & 68.58  \\
  & RTN  & 4 & 128  & 73.16  & 59.04  & 48.38  & 79.25  & 79.11  & 67.79  \\
  & GPTQ  & 4 & 128  & 73.72  & 59.17  & 47.78  & 79.38  & 78.94  & 67.80  \\
  & AWQ & 4 & 128 & 73.01  & 59.43  & 50.00  & 79.55  &  79.22 & 68.24  \\
    \rowcolor[HTML]{D9D9D9} 
  & EfficientQAT & 4 & 128 & 72.53  & 59.43  & 50.94  & 79.84  & 79.43 & 68.43  \\ 
 \midrule
  \multirow{5}{*}{3-70B} & - & 16 &  & 80.51  & 66.36  & 60.41  & 86.99  & 82.37  & 75.33  \\
  & RTN  & 4 & 128  & 78.77  & 65.83  & 57.34  & 85.69  & 82.26  & 73.98  \\
  & GPTQ  & 4 & 128  & 80.51  & 66.12  & 59.04  &  85.77  & 82.26  & 74.74  \\
  & AWQ & 4 & 128 & 80.35  & 65.82  & 59.13  & 86.41  & 82.15  & 74.77  \\
    \rowcolor[HTML]{D9D9D9} 
  & EfficientQAT & 4 & 128 & 79.24   &66.27   & 59.13  & 85.86  & 82.37 & 74.57  \\ 
 \bottomrule
\end{tabular}

\end{table*}
